Multispecies Animal Re-ID Using a Large Community-Curated Dataset

Recent work has established the ecological importance of developing algorithms for identifying animals individually from images. Typically, a separate algorithm is trained for each species, a natural step but one that creates significant barriers to wide-spread use: (1) each effort is expensive, requiring data collection, data curation, and model training, deployment, and maintenance, (2) there is little training data for many species, and (3) commonalities in appearance across species are not exploited. We propose an alternative approach focused on training multi-species individual identification (re-id) models. We construct a dataset that includes 49 species, 37K individual animals, and 225K images, using this data to train a single embedding network for all species. Our model employs an EfficientNetV2 backbone and a sub-center ArcFace loss function with dynamic margins. We evaluate the performance of this multispecies model in several ways. Most notably, we demonstrate that it consistently outperforms models trained separately on each species, achieving an average gain of 12.5% in top-1 accuracy. Furthermore, the model demonstrates strong zero-shot performance and fine-tuning capabilities for new species with limited training data, enabling effective curation of new species through both incremental addition of data to the training set and fine-tuning without the original data. Additionally, our model surpasses the recent MegaDescriptor on unseen species, averaging an 19.2% top-1 improvement per species and showing gains across all 33 species tested. The fully-featured code repository is publicly available on GitHub, and the feature extractor model can be accessed on HuggingFace for seamless integration with wildlife re-identification pipelines. The model is already in production use for 60+ species in a large-scale wildlife monitoring system.

==> abstract_ecoevo.tex <==
\chuck{This the EcoEvo abstract and is here as a placeholder.}

Recent work has established the ecological importance of developing algorithms for identifying animals individually from images. Typically, a separate algorithm is trained for each species, a natural step but one that creates significant barriers to wide-spread use: (1) each effort is expensive, requiring data collection, data curation, and model training, deployment, and maintenance, (2) there is little training data for many species, and (3) commonalities in appearance across species are not exploited.

We propose an alternative approach focused on training multi-species identification models. We start by forming datasets involving clusters of similar species or appearances: cetaceans (23 species), terrestrial carnivores (9), and faces (13). For each we perform experiments to show the potential impact of a multispecies model. We use an embedding model with an EfficientNet backbone and an sub-center ArcFace loss with dynamic margins. First, we compare the performance of species-specific models with a model trained on a cluster of species. Consistent improvement across species establishes immediately the value of a multispecies model. Second, we remove each species in turn from its cluster, train a model on the remaining species, and test ID performance on the held-out species. The third is similar except that after training, the model is fine-tuned on a subset of the held-out species. Different sized subsets are explored. These second and third experiments examine the potential performance of the multispecies model scenario in “bootstrapping” new species — or new viewpoints on known species — with little or no training data.  Experiment results thus far show, e.g. the multispecies cetacean model improves rank-1 performance by nearly 20\% per species, and bootstrapping shows upwards of 90\% of full dataset performance with as low as 5-10\% of the held-out species training data.
\chuck{Some of the foregoing is out of date.}
